A Referable NFT Scheme

Existing NFTs confront restrictions of \textit{one-time incentive} and \textit{product isolation}. Creators cannot obtain benefits once having sold their NFT products due to the lack of relationships across different NFTs, which results in controversial possible profit sharing. This work proposes a referable NFT scheme to extend the incentive sustainability of NFTs. We construct the referable NFT (rNFT) network to increase exposure and enhance the referring relationship of inclusive items. We introduce the DAG topology to generate directed edges between each pair of NFTs with corresponding weights and labels for advanced usage. We accordingly implement and propose the scheme under Ethereum Improvement Proposal (EIP) standards, indexed in EIP-1155. Further, we provide the mathematical formation to analyze the utility for each rNFT participant. The discussion gives general guidance among multi-dimensional parameters. To our knowledge, this is the first study to build the referable NFT network, explicitly showing the virtual connections among NFTs.

==> [CryptEx23] Referable NFT/sections/6-RelatedWork.tex <==

\textbf{NFT Solutions.}

ERC-20R and ERC-721R: Reversible Transactions on Ethereum

https://arxiv.org/pdf/2208.00543.pdf






\textbf{Token Standards. [As of Oct 2, 2022]}

Final:

2981 NFT Royalty Standard

3525 Semi-Fungible Token

4907 Rental NFT, an Extension of EIP-721

4906 EIP-721 Metadata Update Extension

5192 Minimal Soulbound NFTs



Last call: 

5006 Rental NFT, NFT User Extension

5007 Time NFT, EIP-721 Time Extension

5528 Refundable Fungible Token


Review

2135 Consumable NFT for Ticketing

4519 Non-Fungible Tokens Tied to Physical Assets

4799 Non-Fungible Token Ownership Designation Standard

5007 Time NFT, EIP-721 Time Extension

5192 Minimal Soulbound NFTs

4910 Royalty Bearing NFTs

5008 EIP-721 Nonce Extension

5216 EIP-1155 Approval By Amount Extension

5375 NFT Author Information and Consent

5484 Consensual Soulbound Tokens

5496 Multi-privilege Management NFT Extension

5679 Token Minting and Burning




Draft

998 Composable Non-Fungible Token Standard

3569 Sealed NFT Metadata Standard

3754 A Vanilla Non-Fungible Token Standard

4341 Ordered NFT Batch Standard

4353 Interface for Staked Tokens in NFTs

4393 Micropayments Standard for NFTs and Multi Tokens

4494 Permit for ERC-721 NFTs

4521 721/20-compatible transfer

4675 Multi-Fractional Non-Fungible Tokens

4883 Composable SVG NFT

4885 Subscription Token Standard for NFTs and Multi Tokens

4944 Contract with Exactly One Non-fungible Token

4955 Vendor Specific Metadata Extension for Non-Fungible Tokens

5050 Interactive NFTs with Modular Environments

5058 Lockable Non-Fungible Tokens

5173 NFT Future Rewards (nFR)

5185 NFT Updatable Metadata Extension

5218 NFT Rights Management

5334 EIP-721 User And Expires And Level Extension

5380 EIP-721 Entitlement Extension

5409 EIP-1155 Non-Fungible Token extension

5489 NFT Hyperlink Extension

5501 Rental \& Delegation NFT - EIP-721 Extension

5507 Refundable NFTs

5521 Referable NFT

5554 NFT Legal Use, Repurposing, and Remixing

5560 Redeemable NFTs

5570 Digital Receipt Non-Fungible Tokens

5604 NFT Lien

5606 Multiverse NFTs

5625 NFT Metadata JSON Schema dStorage Extension

5633 Composable Soulbound NFT, EIP-1155 Extension

5635 NFT Licensing Agreements

5643 Subscription NFTs




Stagnant 

1633 Re-Fungible Token Standard (RFT)

2615	Non-Fungible Token with mortgage and rental functions

3386	ERC-721 and ERC-1155 to ERC-20 Wrapper	

3440	ERC-721 Editions Standard	

3589 Assemble assets into NFTs

EIP20 \cite{erc20}

EIP721 \cite{erc721}


EIP4907 \cite{erc4907}



\textbf{DAG in Blockchain.}

==> sections/6-RelatedWork.tex <==

\textbf{NFT Solutions.}

ERC-20R and ERC-721R: Reversible Transactions on Ethereum

https://arxiv.org/pdf/2208.00543.pdf






\textbf{Token Standards. [As of Oct 2, 2022]}

Final:

2981 NFT Royalty Standard

3525 Semi-Fungible Token

4907 Rental NFT, an Extension of EIP-721

4906 EIP-721 Metadata Update Extension

5192 Minimal Soulbound NFTs



Last call: 

5006 Rental NFT, NFT User Extension

5007 Time NFT, EIP-721 Time Extension

5528 Refundable Fungible Token


Review

2135 Consumable NFT for Ticketing

4519 Non-Fungible Tokens Tied to Physical Assets

4799 Non-Fungible Token Ownership Designation Standard

5007 Time NFT, EIP-721 Time Extension

5192 Minimal Soulbound NFTs

4910 Royalty Bearing NFTs

5008 EIP-721 Nonce Extension

5216 EIP-1155 Approval By Amount Extension

5375 NFT Author Information and Consent

5484 Consensual Soulbound Tokens

5496 Multi-privilege Management NFT Extension

5679 Token Minting and Burning




Draft

998 Composable Non-Fungible Token Standard

3569 Sealed NFT Metadata Standard

3754 A Vanilla Non-Fungible Token Standard

4341 Ordered NFT Batch Standard

4353 Interface for Staked Tokens in NFTs

4393 Micropayments Standard for NFTs and Multi Tokens

4494 Permit for ERC-721 NFTs

4521 721/20-compatible transfer

4675 Multi-Fractional Non-Fungible Tokens

4883 Composable SVG NFT

4885 Subscription Token Standard for NFTs and Multi Tokens

4944 Contract with Exactly One Non-fungible Token

4955 Vendor Specific Metadata Extension for Non-Fungible Tokens

5050 Interactive NFTs with Modular Environments

5058 Lockable Non-Fungible Tokens

5173 NFT Future Rewards (nFR)

5185 NFT Updatable Metadata Extension

5218 NFT Rights Management

5334 EIP-721 User And Expires And Level Extension

5380 EIP-721 Entitlement Extension

5409 EIP-1155 Non-Fungible Token extension

5489 NFT Hyperlink Extension

5501 Rental \& Delegation NFT - EIP-721 Extension

5507 Refundable NFTs

5521 Referable NFT

5554 NFT Legal Use, Repurposing, and Remixing

5560 Redeemable NFTs

5570 Digital Receipt Non-Fungible Tokens

5604 NFT Lien

5606 Multiverse NFTs

5625 NFT Metadata JSON Schema dStorage Extension

5633 Composable Soulbound NFT, EIP-1155 Extension

5635 NFT Licensing Agreements

5643 Subscription NFTs




Stagnant 

1633 Re-Fungible Token Standard (RFT)

2615	Non-Fungible Token with mortgage and rental functions

3386	ERC-721 and ERC-1155 to ERC-20 Wrapper	

3440	ERC-721 Editions Standard	

3589 Assemble assets into NFTs

EIP20 \cite{erc20}

EIP721 \cite{erc721}


EIP4907 \cite{erc4907}



\textbf{DAG in Blockchain.}
